Stagnation of block GMRES and its relationship to block FOM

We analyze the the convergence behavior of block GMRES and characterize the phenomenon of stagnation which is then related to the behavior of the block FOM method. We generalize the block FOM method to generate well-defined approximations in the case that block FOM would normally break down, and these generalized solutions are used in our analysis. This behavior is also related to the principal angles between the column-space of the previous block GMRES residual and the current minimum residual constraint space. At iteration $j$, it is shown that the proper generalization of GMRES stagnation to the block setting relates to the columnspace of the $j$th block Arnoldi vector. Our analysis covers both the cases of normal iterations as well as block Arnoldi breakdown wherein dependent basis vectors are replaced with random ones. Numerical examples are given to illustrate what we have proven, including a small application problem to demonstrate the validity of the analysis in a less pathological case.

==> fourStagAnalysis.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.35]{fourStagAnalysis1.pdf}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{\label{figure.fourStagAnalysis} Relative two-norm residual curves for stagnating  block GMRES and block FOM for the $30\times 30$ shift matrix. The black solid and dashed curves correspond respectively to the  block FOM and GMRES residuals for the first right-hand side.  Similarly,  the gray solid and dashed curves, respectively, correspond to the second right-hand side.}
\end{figure}



==> sherman4Analysis.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.25]{sherman4Analysis1.pdf}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{\label{figure.sherman4Analysis} In the left-hand figure, we have the $2$-norm residual curves of block GMRES and FOM for a linear  system with two right-hand sides using the {\tt sherman4 } matrix from \cite{DH.2011}. In the right-hand figure, we have the squares of the sines $\curl{s_{1}^{2},s_{2}^{2}}$ coming from the  orthogonal transformations as discussed in the our analysis.  We have marked four points  in both figures so that the reader may compare convergence behavior with sine-squared values.}
\end{figure}



==> sherman4Conv.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.35]{sherman4Conv1.pdf}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{\label{figure.sherman4Conv} Relative two-norm residual curves for  block GMRES and block FOM applied to the $1104\times 1104$ {\tt sherman4} matrix {\rm \cite{DH.2011}}. The black solid and dashed curves correspond respectively to the  block FOM and GMRES residuals for the first right-hand side.  Similarly,  the gray solid and dashed curves, respectively, correspond to the second right-hand side.}
\end{figure}


